SIGL: Securing Software Installations Through Deep Graph Learning

Many users implicitly assume that software can only be exploited after it is installed. However, recent supply-chain attacks demonstrate that application integrity must be ensured during installation itself. We introduce SIGL, a new tool for detecting malicious behavior during software installation. SIGL collects traces of system call activity, building a data provenance graph that it analyzes using a novel autoencoder architecture with a graph long short-term memory network (graph LSTM) for the encoder and a standard multilayer perceptron for the decoder. SIGL flags suspicious installations as well as the specific installation-time processes that are likely to be malicious. Using a test corpus of 625 malicious installers containing real-world malware, we demonstrate that SIGL has a detection accuracy of 96%, outperforming similar systems from industry and academia by up to 87% in precision and recall and 45% in accuracy. We also demonstrate that SIGL can pinpoint the processes most likely to have triggered malicious behavior, works on different audit platforms and operating systems, and is robust to training data contamination and adversarial attack. It can be used with application-specific models, even in the presence of new software versions, as well as application-agnostic meta-models that encompass a wide range of applications and installers.

==> availability.tex <==
To perform further evaluation against the StreamSpot~\cite{manzoor2016fast} algorithm (\autoref{sec:evaluation}),
 we re-implemented StreamSpot and made the code available online at \emph{anonymized}.

==> detailed_comparison.tex <==
We show detailed experiment results for Frappuccino (\autoref{table:eval:results:frappuccino})
and StreamSpot (\autoref{table:eval:results:streamspot:original}, \autoref{table:eval:results:streamspot:reimp}).
We discuss these results in \autoref{eval:results:comparison}.

\begin{table}[ht!]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l | c c c c}
	Software Installer & Precision & Recall & Accuracy & F-Score \\ %& \# of FP & \# of FN\\
	\hline\hline
	FireFox & 1.0 & 0.1 & 0.59 & 0.18 \\%& 0 & 18 \\
	%\hline
	%ThunderBird  \\ %& 0 & 18\\
	\hline
	FileZilla & 1.0 & 0.48 & 0.67 & 0.65 \\ %& 0 & 21\\
	\hline
	PWSafe & N/A & 0 & 0.38 & N/A \\ %& 0 & 40\\
	\hline
	MP3Gain & 1.0 & 0.03 & 0.38 & 0.05 \\ %& 0 & 39 \\
 	\hline
	ShotCut & N/A & 0 & 0.38 & N/A \\ %& 0 & 40\\
	\hline
	TeamViewer & 0 & 0 & 0.34 & N/A \\ %& 2 & 40\\
	\hline
	Foobar & 1.0 & 0.28 & 0.55 & 0.44 \\ %& 0 & 29\\
	\hline
	7Zip & N/A & 0 & 0.38 & N/A \\ %& 0 & 40\\
	\hline
	TurboVNC & N/A & 0 & 0.38 & N/A \\%& 0 & 40\\
	\hline
	WinMerge & 0.97 & 0.83 & 0.87 & 0.89 \\ %& 1 & 7\\
	\hline
	Launchy & N/A & 0 & 0.51 & N/A \\ %& 0 & 40 \\
	\hline
	Skype & 0 & 0 & 0.34 & N/A \\ %& 1 & 40\\
	\hline
	WinRAR & N/A & 0 & 0.55 & N/A \\ %& 0 & 20\\
	\hline
	DropBox  & 1.0 & 0.05 & 0.56 & 0.1 \\%& 0 & 19 \\
	\hline 
	Slack & 1.0 & 0.05 & 0.57 & 0.1 \\ %& 0 & 19\\
	\hline
	Flash & 1.0 & 0.2 & 0.64 & 0.33 \\ %& 0 & 16\\
	\hline
	OneDrive & N/A & 0 & 0.55 & N/A \\ %& 0 & 20\\
	\hline
	NotePad++ & N/A & 0 & 0.53 & N/A  \\ %& 0 & 20\\
	\hline
	Adobe Acrobat Reader & 0 & 0 & 0.5 & N/A \\ %& 3 & 20\\
	\hline
	ICBC Anti-Phishing & N/A & 0 & 0.53 & N/A \\ %& 0 & 20\\
	\hline
	ESET AV Remover & N/A & 0 & 0.51 & N/A \\%& 0 & 20 \\
	\hline\hline
\end{tabular}
}
\caption{Frappuccino result breakdown for each software installer. }
\label{table:eval:results:frappuccino}
\end{table}

\newpage

\begin{table}[ht!]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l | c c c c}
	Software Installer & Precision & Recall & Accuracy & F-Score \\ %& \# of FP (1/2/3 Hops) & \# of FN (1/2/3 Hops) \\
	\hline\hline
	FireFox & N/A & 0 & 0.55 & N/A \\%& 0/0/0 & 20/18/20 \\
	%\hline
	%ThunderBird & 1.0 & 0.8 & 0.91 & 0.89 \\ %& 0/0/1 & 20/4/19\\
	\hline
	FileZilla & N/A & 0 & 0.38 & N/A \\ %& 0/0/1 & 40/38/2\\
	\hline
	PWSafe & N/A & 0 & 0.38 & N/A \\ %& 0/0/0 & 40/33/12\\
	\hline
	MP3Gain & N/A & 0 & 0.37 & N/A \\%& 0/0/0 & 40/36/0 \\
 	\hline
	ShotCut & N/A & 0 & 0.38 & N/A \\ %& 0/1/0 & 40/40/39\\
	\hline
	TeamViewer & N/A & 0 & 0.38 & N/A\\ %& 0/0/1 & 40/39/37\\
	\hline
	Foobar & N/A & 0 & 0.38 & N/A\\ %& 0/0/0 & 40/38/34\\
	\hline
	7Zip & N/A & 0 & 0.38 & N/A \\ %& 0/0/0 & 40/38/22\\
	\hline
	TurboVNC & N/A & 0 & 0.38 & N/A\\%& 0/1/0 & 40/28/15\\
	\hline
	WinMerge & N/A & 0 & 0.37 & N/A \\ %& 0/0/1 & 40/33/20\\
	\hline
	Launchy  & N/A & 0 & 0.51 & N/A\\ %& 0/3/0 & 40/13/35\\
	\hline
	Skype & N/A & 0 & 0.35 & N/A \\ %& 0/0/1 & 40/40/23\\
	\hline
	WinRAR & N/A & 0 & 0.55 & N/A \\ %& 0/0/2 & 20/20/17\\
	\hline
	DropBox & N/A & 0 & 0.53 & N/A \\ %& 0/0/2 & 20/0/0\\
	\hline 
	Slack & N/A & 0 & 0.55 & N/A \\ %& 0/0/0 & 20/3/12\\
	\hline
	Flash & N/A & 0 & 0.55 & N/A\\ %& 0/0/0 & 20/20/6\\
	\hline
	OneDrive & N/A & 0 & 0.55 & N/A\\ %& 0/0/1 & 20/8/18\\
	\hline
	NotePad++ & N/A & 0 & 0.53 & N/A \\ %& 0/0/0 & 20/15/0\\
	\hline
	Adobe Acrobat Reader & N/A & 0 & 0.57 & N/A \\ %& 0/0/0 & 20/19/20\\
	\hline
	ICBC Anti-Phishing & 0.87 & 0.65 & 0.79 & 0.74 \\ %& 2/2/0 & 7/7/18\\
	\hline
	ESET AV Remover & N/A & 0 & 0.51 & N/A \\%& 0/0/0 & 20/20/20 \\
	\hline\hline
\end{tabular}
}
\caption{StreamSpot (original one-hop implementation) result breakdown for each software installer. }
\label{table:eval:results:streamspot:original}
\end{table}

%\newpage

\begin{table}[ht!]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l | c c c c}
	Software Installer & Precision & Recall & Accuracy & F-Score \\ %& \# of FP (1/2/3 Hops) & \# of FN (1/2/3 Hops) \\
	\hline\hline
	FireFox & 1.0 & 0.1 & 0.59 & 0.18 \\%& 0/0/0 & 20/18/20 \\
	%\hline
	%ThunderBird & 1.0 & 0.8 & 0.91 & 0.89 \\ %& 0/0/1 & 20/4/19\\
	\hline
	FileZilla & 0.97 & 0.95 & 0.95 & 0.96 \\ %& 0/0/1 & 40/38/2\\
	\hline
	PWSafe & 1.0 & 0.7 & 0.81 & 0.82 \\ %& 0/0/0 & 40/33/12\\
	\hline
	MP3Gain & 1.0 & 1.0 & 1.0 & 1.0 \\%& 0/0/0 & 40/36/0 \\
 	\hline
	ShotCut & 1.0 & 0.03 & 0.39 & 0.05 \\ %& 0/1/0 & 40/40/39\\
	\hline
	TeamViewer & 0.75 & 0.08 & 0.41 & 0.14\\ %& 0/0/1 & 40/39/37\\
	\hline
	Foobar & 1.0 & 0.15 & 0.47 & 0.26\\ %& 0/0/0 & 40/38/34\\
	\hline
	7Zip & 1.0 & 0.45 & 0.66 & 0.62 \\ %& 0/0/0 & 40/38/22\\
	\hline
	TurboVNC & 1.0 & 0.63 & 0.77 & 0.77\\%& 0/1/0 & 40/28/15\\
	\hline
	WinMerge & 0.95 & 0.5 & 0.67 & 0.66 \\ %& 0/0/1 & 40/33/20\\
	\hline
	Launchy  & 0.9 & 0.68 & 0.80 & 0.77\\ %& 0/3/0 & 40/13/35\\
	\hline
	Skype & 0.94 & 0.43 & 0.61 & 0.59 \\ %& 0/0/1 & 40/40/23\\
	\hline
	WinRAR & 0.6 & 0.15 & 0.57 & 0.24 \\ %& 0/0/2 & 20/20/17\\
	\hline
	DropBox & 1.0 & 1.0 & 1.0 & 1.0 \\ %& 0/0/2 & 20/0/0\\
	\hline 
	Slack & 1.0 & 0.85 & 0.93 & 0.92 \\ %& 0/0/0 & 20/3/12\\
	\hline
	Flash & 1.0 & 0.7 & 0.86 & 0.82\\ %& 0/0/0 & 20/20/6\\
	\hline
	OneDrive & 1.0 & 0.6 & 0.82 & 0.75\\ %& 0/0/1 & 20/8/18\\
	\hline
	NotePad++ & 1.0 & 1.0 & 1.0 & 1.0 \\ %& 0/0/0 & 20/15/0\\
	\hline
	Adobe Acrobat Reader & 1.0 & 0.05 & 0.59 & 0.10 \\ %& 0/0/0 & 20/19/20\\
	\hline
	ICBC Anti-Phishing & 0.87 & 0.65 & 0.79 & 0.74 \\ %& 2/2/0 & 7/7/18\\
	\hline
	ESET AV Remover & N/A & 0 & 0.51 & N/A \\%& 0/0/0 & 20/20/20 \\
	\hline\hline
\end{tabular}
}
\caption{StreamSpot (reimplementation with larger graph neighborhood exploration) result breakdown for each software installer. }
\label{table:eval:results:streamspot:reimp}
\end{table}


==> lstm.tex <==
The long short-term memory network (LSTM)~\cite{hochreiter1997long},
a specific type of recurrent neural network (RNN),
is a popular machine learning model used to 
capture long-term dependencies of linear sequences.
Although originally developed for NLP-related tasks
(\eg machine translation~\cite{bahdanau2014neural} and speech recognition~\cite{graves2013hybrid}),
LSTMs have been successfully adapted to a variety of
sequence modeling and prediction tasks,
such as image caption generation~\cite{vinyals2015show},
program execution~\cite{zaremba2014learning},
and attack prediction~\cite{shen2018tiresias}.

The standard LSTM architecture learns
sequential information propagation only;
tree-structured LSTMs~\cite{tai2015improved}
and the more general graph LSTMs~\cite{peng2017cross}
are two natural extensions that incorporate richer network topologies.
% They are originally designed for complex NLP tasks 
% that analyze tree representations of sentences and
% extract cross-sentence relations with intra- and inter-sentential dependencies~\cite{peng2017cross}.
Graph LSTMs
allow for flexible graph structures (\eg DAGs) and consider distinct edge types.
%\notems{Is it correct to say "As in standard neural networks"}
As in standard LSTMs,
each graph LSTM unit $j$ contains
input and output gates $i_{j}$ and $o_{j}$,
a memory cell $c_{j}$, 
and the hidden state $h_{j}$.
A graph LSTM unit might have multiple child units $C(j)$.
For each child unit $k$,
there is a forget gate $f_{jk}$ and a type-specific weight matrix $U^{e_{jk}}$,
where $e_{jk}$ denotes the edge type that connects $j$ and $k$.
%\notems{I wonder if this is useful or if it might be better to give
%some intuition about the transitions?}
Given the input vector for unit $j$, the transition equations are~\cite{peng2017cross}:
\begin{align}
i_{j} &= \sigma(W_{i}x_{j} + \sum_{k\in C(j)}U_{i}^{e_{jk}}h_{k} + b_{i}) \nonumber \\
o_{j} &= \sigma(W_{o}x_{j} + \sum_{k\in C(j)}U_{o}^{e_{jk}}h_{k} + b_{o}) \nonumber \\
\tilde{c_{j}} &= tanh(W_{c}x_{j} + \sum_{k\in C(j)}U_{c}^{e_{jk}}h_{k} + b_{c}) \nonumber \\
f_{jk} &= \sigma(W_{f}x_{j} + U_{f}^{e_{jk}}h_{k} + b_{f}) \nonumber \\
c_{j} &= i_{j} \odot \tilde{c_{j}} + \sum_{k\in C(j)}f_{jk} \odot c_{k} \nonumber \\
h_{j} &= o_{j} \odot tanh(c_{j}) \nonumber
\end{align}
where $x_{j}$ is the input feature vector,
$W$'s are the input weight matrices,
$b$'s are the bias vectors,
$\sigma$ is the sigmoid function,
$tanh$ is the hyperbolic tangent function,
and $\odot$ is the Hadamard product.


==> major_revision.tex <==
We address all of the reviewer concerns in the major revision as follows:
\begin{itemize}[leftmargin=*]
	\setlength\itemsep{0em}
	
	\item We discuss (in~\autoref{sec:discussion}) and evaluate (in~\autoref{eval:results:adversarial}) adversarial scenarios 
	to demonstrate \system's robustness against attack evasion. We show that it is difficult to circumvent \system's detection
	approach. (Reviewer A, B \& C)
	
	\item We provide false positive (FP) percentage in~\autoref{table:eval:results:overall} and the absolute number of FPs
	we encountered in our enterprise in~\autoref{eval:results:comparison} and 
	in our experimental testbed in~\autoref{eval:results:linux} where additional experiments were performed. 
	We also discuss its implications in~\autoref{eval:results:comparison}. We show that the number of FPs is manageable.
	In fact, it is dramatically reduced compared to the commercial TDS used by the enterprise. 
	We also evaluated \system when it is trained on a diverse benign dataset in~\autoref{eval:results:meta} 
	and~\autoref{eval:results:linux}. (Reviewer A, D, \& E)
	
	\item We discuss how training data can be obtained in~\autoref{sec:discussion}.
	Additionally, we evaluate \system's robustness against data contamination in~\autoref{eval:results:contamination}. 
	Per reviewers' suggestions, we performed a controlled experiment where the training data is deliberately contaminated
	to understand the impact on detection performance. We show that \system is robust to data contamination.
	(Reviewer A \& B)
	
	\item We provide more details on how the installation graph is marked as anomalous in~\autoref{sec:framework:detection}. (Reviewer E)
	
	\item We evaluate \system's ability to build meta-models in~\autoref{eval:results:meta}.
	We show that \system maintains high detection performance with meta-models. (Reviewer D)
	
	\item We evaluate in~\autoref{eval:results:linux} \system's ability to detect malicious installers even when no malware binary is written to disk.
	We show that \system can detect malicious execution without malware creating any binary execution file. (Reviewer A \& E)
	
	\item We show in~\autoref{eval:results:linux} that \system does not need to build application-specific models to detect malicious installers;
	it can learn generalized benign installation behavior that is application-agnostic.
	We evaluate \system with a large variety of software and on different OS platforms and installation frameworks. (Reviewer C \& D)
	
	\item We provide more details on how node embeddings are constructed from directed random walk in~\autoref{sec:framework:embedding}. (Reviewer E)
	
\end{itemize}
